Deformable 3D Gaussian Splatting for Animatable Human Avatars

Recent advances in neural radiance fields enable novel view synthesis of photo-realistic images in dynamic settings, which can be applied to scenarios with human animation. Commonly used implicit backbones to establish accurate models, however, require many input views and additional annotations such as human masks, UV maps and depth maps. In this work, we propose ParDy-Human (Parameterized Dynamic Human Avatar), a fully explicit approach to construct a digital avatar from as little as a single monocular sequence. ParDy-Human introduces parameter-driven dynamics into 3D Gaussian Splatting where 3D Gaussians are deformed by a human pose model to animate the avatar. Our method is composed of two parts: A first module that deforms canonical 3D Gaussians according to SMPL vertices and a consecutive module that further takes their designed joint encodings and predicts per Gaussian deformations to deal with dynamics beyond SMPL vertex deformations. Images are then synthesized by a rasterizer. ParDy-Human constitutes an explicit model for realistic dynamic human avatars which requires significantly fewer training views and images. Our avatars learning is free of additional annotations such as masks and can be trained with variable backgrounds while inferring full-resolution images efficiently even on consumer hardware. We provide experimental evidence to show that ParDy-Human outperforms state-of-the-art methods on ZJU-MoCap and THUman4.0 datasets both quantitatively and visually.

==> sec/old/old_2_related.tex <==
\section{Related Work}
\label{sec:related_work}
\ben{let's shrink this heavily! and include \cite{yang2023deformable3dgs}}
\subsection{View Synthesis of 3D Scenes}
3D scenes are represented in the literature in a plethora of different ways. Classical explicit representations include point clouds, voxels, and meshes, while classical \textbf{implicit representations} utilize signed distance fields (SDFs). Historical approaches involve lightfield interpolations~\cite{szeliski1996lumigraph,levoy1996lightfield} and volumetric representations in the form of coloured voxel grids~\cite{szeliski1998stereo,seitz1999photorealistic}. Implicit neural representations leverage neural networks to encode the scene. Occupancy networks learn 3D reconstruction in function space~\cite{Mescheder2019occupancy} and DeepSDFs represent the scene with a learned SDF~\cite{Park2019deepsdf}. \textbf{Neural Radiance Fields (NeRFs)} are a recent advancement in 3D scene representation that utilizes neural networks to model the volumetric properties and appearance of scenes~\cite{mildenhall2021nerf,muller2022instant,barron2022mip}. They have become very popular due to their ability for high-fidelity novel view synthesis.

Accurate camera poses is crucial to train NeRFs. Typically, camera poses are derived from structure-from-motion techniques like COLMAP~\cite{schoenberger2016sfm}. Typically only COLMAP's camera poses are used despite the potential of its co-derived distance estimates~\cite{jung2023importance} to enhance convergence~\cite{roessle2022dense,deng2022depth}. Methods like BARF~\cite{lin2021barf}, Nerf--~\cite{wang2021nerf}, and PoseDiffusion~\cite{wang2023posediffusion} can robustify camera pose retrieval, but they fail in case of scene deformations. Dynamic SLAM techniques~\cite{karaoglu2023dynamon} offer a solution by segmenting the scene into static and deformable components.
In line with existing literature~\cite{park2021nerfies,li2022neural,weng2022humannerf,chen2023uv}, we adopt the convention of assuming either static cameras or posed images to learn our 3D representation.

Very recently, \textbf{3D Gaussian splatting} has emerged as a compelling \textbf{explicit method} to represent 3D scenes~\cite{kerbl20233d}. This technique capitalizes on the co-produced COLMAP point cloud to represent the scene using 3D Gaussians, optimizing their anisotropic covariance and incorporating visibility-aware rendering. This approach not only expedites training but also enables real-time rendering of unbounded and complete scenes with exceptional quality.
The method has further been extended in time~\cite{wu20234d} by representing generic 4D scenes and leveraging temporal connections between adjacent Gaussians to facilitates real-time rendering of dynamic scenes. Additionally, 3D Gaussians can be densely tracked over time~\cite{luiten2023dynamic}. In our work, we take a different approach, utilizing a deformation field in conjunction with a parametric human model. This allows us to associate dynamic 3D Gaussians in a canonical representation, enabling the high-fidelity learning of a 3D human avatar that can be freely animated using its underlying parametric model.

\subsection{Dynamic Scene Representations}
Dynamic scenes are also considered both to render novel camera views and to stream content in real-time. Carranza et al.~\cite{carranza2003free} present a free-viewpoint video of human actors, enabling interactive 3D observation of dynamic real-world scenes and Starck et al.~\cite{starck2007surface} leverage skeletal motion for marker-free reconstruction of humans. A series of works by researchers from Microsoft~\cite{collet2015high,dou2016fusion4d,orts2016holoportation} introduce high-quality streamable free-viewpoint systems to enable real-time content-agnostic scene transfer to facilitate AR/VR telepresence with multi-view RGBD stereo setups.

Deformable 3D scene are represented by neural volumes optimized from 2D data through an encoder-decoder framework using differentiable ray marching~\cite{lombardi2019neural} and volumetric primitives are used to render more efficiently~\cite{lombardi2021mixture}.
Also NeRFs have been extended to the temporal domain with time-conditioned features and keyframe-based training for neural 3D video synthesis from \textbf{multi-view} video~\cite{li2022neural}. D-NeRF~\cite{pumarola2021d} explores the deformable multi-view scenarios using an implicit 3D deformation fields to correlate ray features through time.

While these methods rely on synchronized multi-view setups, Nerfies~\cite{park2021nerfies} addresses the challenging case of a \textbf{moving monocular camera} with limited scene dynamics as video input and optimizes a 5D NeRF with a deformation field incorporating an elastic regularizer for robustness.
In a similar vein, they introduced HyperNeRF~\cite{park2021hypernerf}, offering a higher-dimensional representation that also accounts for topological changes.
Li et al.~\cite{li2021neural} further design Neural Scene Flow Fields for space-time view synthesis of dynamic scenes, modeling dynamics as a continuous function of appearance, geometry, and 3D scene motion leading to applications on in-the-wild videos including thin structures.

Deformable scenes with NeRFs can be efficiently played or replayed from various perspectives using techniques such as NeRFPlayer~\cite{Song2023nerfplayer} which decomposes the 4D scene into static, deforming, and newly appearing regions, each represented by a separate neural field. The recent proposal 4K4D~\cite{xu20234k4d}, in turn, leverages a 4D point cloud representation along with hardware rasterization With depth peeling to achieves over 400 frames per second (FPS) at 1080p resolution on an RTX 4090 GPU.

While all these \textbf{scene-agnostic} approaches demonstrate effectiveness in blending rays into canonical spaces, they may suffer from depth ambiguities arising from monocular depth, manifesting as visual floaters in the free space for novel views further away from observations which can be overcome using human-aware 3D models.

\subsection{Humans in 3D}
The representation of humans in 3D space has seen significant advancements through the development and extension of spatial human body models in the past decade. Early methods focused on predicting keypoints and skeletons for major body joints~\cite{insafutdinov2016deepercut}. These models have since evolved to incorporate finer details, including hand, face, and foot keypoints~\cite{openpose}. Notably, with SMPL~\cite{loper2015smpl} a widely adopted \textbf{volumetric representation} has been introduced, utilizing skinning techniques and blend shapes optimized on real 3D body scans, providing realistic representations for non-clothed humans. The SMPL-X~\cite{SMPL-X:2019} model further refines this by integrating the FLAME~\cite{flame} head model and MANO~\cite{mano} hand model. STAR~\cite{osman2020star} has further improved the model and provides more realistic deformation while reducing the model parameters. In practice, these model parameters can be directly predicted or correspondences to map all 2D pixels of a segmented human body onto its 3D surface are established~\cite{guler2018densepose}.

These advancements have been paralleled by substantial efforts in dataset acquisition, leveraging advanced hardware setups, accurate annotations, and synchronized multi-view capture. Early work by Kanade et al.~\cite{kanade1997virtualized} utilized a multi-camera dome for reconstruction. Subsequent popular datasets like like Human3.6M~\cite{ionescu2013human3p6} build on these experiences and provide eleven human captures with four high-resolution 1MP cameras while ZJU-Mocap~\cite{peng2021neural} features nine humans with 21 cameras of 1MP reach, significantly expanding the available resources and THUman4.0~\cite{zheng2022structured} leverages even 24 cameras at 30 FPS with three human subjects.
The ActorsHQ dataset~\cite{icsik2023humanrf} represents a recent milestone towards high fidelity data, comprising eight human captures with an impressive array of 160 surround view cameras, each operating at 12 MP resolution and 25 FPS. This setup, supported by 420 synchronized LEDs and various lenses, ensures impeccable illumination and field of view. However, it is important to note that even with advanced hardware, obtaining high-quality 3D annotations remains a costly endeavor~\cite{wang2022phocal,jung2022housecat6d,icsik2023humanrf}.

In the context of registering 3D shapes, \textbf{scene-agnostic} methods typically rely on point cloud descriptors~\cite{drost2010model,rusu20113d,salti2014shot,guo2020deep} that can be used for both 3D and 4D descriptor matching~\cite{deng2018ppfnet,yu2021cofinet,qin2022geometric,saleh2022bending,yu2023rotation}, or on functional maps applied to known shapes~\cite{litany2017deep,bastian2023s3m}. Establishing the connection to mentioned parametric models and finding correspondences to canonical parts of them plays a crucial role in enabling subsequent 3D avatar animation.

\subsection{Animatable Human Avatars}
The pursuit of animatable human avatars has seen a progression from static 3D human surface recovery to more intricate neural approaches guided by 3D human models. Methods like PiFu~\cite{saito2019pifu} and PiFuHD~\cite{saito2020pifuhd} adeptly recover static 3D humans from single images through pixel-aligned implicit functions, enabling high-resolution digitization of individuals.
The techniques of Deepcap~\cite{habermann2020deepcap} focus on deformable pre-scanned humans for monocular human performance capture, leveraging weak multi-view supervision, while Monoperfcap~\cite{xu2018monoperfcap} provided the first marker-less method for temporally coherent 3D performance capture of a clothed human from monocular video.

The emergence of neural methods specializing in human rendering marked a significant shift. Models like Neural Body~\cite{pumarola2021d} optimize latent features for each mesh vertex, leveraging an SMPL model. Approaches, including Neural Articulated Radiance Field~\cite{noguchi2021neural}, A-NeRF~\cite{su2021nerf}, and TAVA~\cite{li2022tava} provide solutions to learn human shape, appearance, and pose leveraging skeleton input.
PoseVocab~\cite{li2023posevocab} further learns an optimal pose embedding for dynamic human motion from multi-view RGB by factorizing global pose into embeddings for each joint together with a strategy to interpolate features for fine-grained human appearance.

For monocular video, Selfrecon~\cite{jiang2022selfrecon} combines explicit and implicit representations using SDFs for 3D human body representations while NeuMan~\cite{jiang2022neuman} splits the scene content to train two NeRFs for static background and human. Animatable NeRF~\cite{peng2021animatable} and HumanNerf~\cite{weng2022humannerf} integrates motion priors in the form of SMPL~\cite{loper2015smpl} parameters to regularize field prediction.
The canonical representation is warped into the target frame by Arah~\cite{wang2022arah}, SNARF~\cite{chen2021snarf} as well as Scanimate~\cite{saito2021scanimate} while other methods~\cite{liu2021neural,xu2022surface} use backward sampling from the observation.
MonoHuman~\cite{Yu_2023_CVPR} models deformation bi-directionally to retrieve view-consistent avatars.
Additionally, they leverage a motion diffusion model~\cite{tevet2023human} to generate realistic pose sequences for character animation.
Typically garment deformation is tied to the model, however, Zheng et al.~\cite{zheng2022structured} use a residual model correction to fit dynamic cloth deformations with local fields attached to pre-defined SMPL nodes.
Inherent limitations in texture fidelity have addressed with generative models using adversarial approaches~\cite{wang2021towards} and latent diffusion models~\cite{svitov2023dinar}.

All these approaches prioritize rendering quality but also grapple with high computational costs for both training and testing. NeRFs are great to mimic visual appearance even when geometry is fixed~\cite{chen2023texpose}. UV Volumes~\cite{chen2023uv} leverages this to establish an efficient rendering pipeline for human avatars using 2D-3D correspondences as used in other domains~\cite{li2023nerf}, significantly expediting the process. InstantAvatar~\cite{jiang2023instantavatar} efficiently builds avatars using recent acceleration techniques~\cite{muller2022instant,chen2023fast}.

The popularity of implicit neural fields for scene representations has accelerated progress in this domain and undoubtedly lead to impressive results. However, these methods inherently struggle to represent empty space efficiently and acceleration is limited by efficient sampling for ray-marching and the structured representations of the scene.
Using explicit 3D Gaussians allows us to overcome these bottlenecks with an unstructured representation for more efficient training with higher quality and faster inference speed.





